Towards Distributed Coevolutionary GANs

Generative Adversarial Networks (GANs) have become one of the dominant methods for deep generative modeling. Despite their demonstrated success on multiple vision tasks, GANs are difficult to train and much research has been dedicated towards understanding and improving their gradient-based learning dynamics. Here, we investigate the use of coevolution, a class of black-box (gradient-free) co-optimization techniques and a powerful tool in evolutionary computing, as a supplement to gradient-based GAN training techniques. Experiments on a simple model that exhibits several of the GAN gradient-based dynamics (e.g., mode collapse, oscillatory behavior, and vanishing gradients) show that coevolution is a promising framework for escaping degenerate GAN training behaviors.

==> ec4ml.tex <==
\paragraph{Evolutionary Computing for Machine Learning.} Combined with sufficient computing resources and data, evolutionary algorithms have shown to rival the performance of gradient-based techniques for several machine learning problems. By evaluating population individuals only on a small number of training examples per generation, Morse et al.~\cite{morse2016simple} showed that a simple evolutionary algorithm can optimize neural networks of over $1000$ dimensions as effectively as gradient descent algorithms. A team from \textsf{OpenAI}~\cite{salimans2017evolution} applied a simplified version of Natural Evolution Strategies~(NES)~\cite{wierstra2008natural} with a novel communication strategy to a collection of reinforcement learning (RL) benchmark problems. Due to better parallelization over thousand cores, they achieved much faster training times (wall-clock time) than popular RL techniques. Likewise, a team from~\textsf{Uber~AI}~\cite{clune2017uber}
%\cite{such2017deep, conti2017improving}
 showed that deep convolutional networks with over $4$ million parameters trained with genetic algorithms can also reach results competitive to those trained with \textsf{OpenAI}'s NES and other RL algorithms. \textsf{OpenAI} ran their experiments on a computing cluster of $80$ machines and $1440$ CPU cores~\cite{salimans2017evolution}, whereas \textsf{Uber~AI} employed a range of hundreds to thousands of CPU cores (depending on availability). %EC-Star~\cite{hodjat2014maintenance} is another example of a large scale evolutionary computation system.

==> theory.tex <==

\paragraph{Theoretical Connections.}  In the context of zero-sum games, the Nash Equilibrium solution concept is an appropriate choice in coevolution literature when $\calU$ and $\calV$ are finite~\cite{popovici2012coevolutionary,ficici2003game,oliehoek2006parallel}. It operates over mixtures of components $\{\calS_u \}$ and $\{\calS_v\}$. For continuous $\calU$ and $\calV$, Algorithm~\ref{alg:adv-coev-gan} shares a similar setup to the framework presented in~\cite{arora2017generalization}, where it was shown that a finite mixture of generators can win against all discriminators. 
%In particular, let $\calS_u$ be a distribution supported on $\calU$ and $\calS_v$ be a distribution supported on $\calV$. 
If both the generator and discriminator are allowed to play mixed strategies, i.e., sample $u\sim \calS_u$, $v\sim \calS_v$ every time they play. Then a minimax solution can be obtained. Instead of infinite mixture,~Arora et al.~\cite{arora2017generalization} show that an $\epsilon$-approximate equilibrium can be obtained with mixture of finitely many generators and discriminators (see~\cite[Definition 3 and Theorem 4.2]{arora2017generalization}). 
\begin{comment}

For sake of completeness, we reproduce the supporting definition and the aforementioned statement (theorem).

\begin{definition}[$\epsilon$-approximate equilibrium~\cite{arora2017generalization}]
	\label{def:approx-equilbrium} 
	A pair of mixed strategies ($\calS_u, \calS_v$) is an $\epsilon$-approximate equilibrium, if for some value $V$,
	\begin{eqnarray}
	\forall u \in \calU\;, \E_{v\sim \calS_v} [\calL(u,v)] \geq V - \epsilon \;, \nonumber\\
	\forall v \in \calV\;, \E_{u\sim \calS_u} [\calL(u,v)] \leq V + \epsilon\;. \nonumber
	\end{eqnarray}
	If the strategies $\calS_u, \calS_v$ are pure strategies, then this pair is called an $\epsilon$-approximate pure equilibrium.
\end{definition}



\begin{theorem}[Arora et al.~\cite{arora2017generalization}] Assume that $\phi$ is $L_\phi$-Lipschitz and bounded in $[-\triangle, \triangle]$, the generators and discriminators are $L$-Lipschitz with respect to their parameters and $L^\prime$-Lipschitz with respect to their inputs, then if the generator can approximate any point mass, there is a universal constant $C>0$ such that for any $\epsilon$, there exists $T=\frac{C\triangle^2 p \log(LL^\prime L_\phi p / \epsilon)}{\epsilon^2}$~generators~$G_{u_1}, \ldots, G_{u_T}$. Let $\calS_u$ be a uniform distribution on $u_i$, and $D$ is a discriminator that outputs only $\frac{1}{2}$, then $(\calS_u, D)$ is an $\epsilon$-approximate equilibrium.
\end{theorem}

\end{comment}
\cite[Theorem 4.2]{arora2017generalization} guarantees existence of approximate equilibrium using a mixture of not too many generators and discriminators. Using a mixture of $N$ components (generators and discriminators), Arora et al.~\cite{arora2017generalization} formulate their training objective as
\begin{equation}
\label{eq:mix-gan}
\min_{\{u_i\}, \{w_{u_i}\}} \max_{\{v_j\}, \{w_{v_j}\}} \sum^{N}_{i=1} \sum^{N}_{j=1} w_{u_i}w_{w_{v_j}} \calL(u_i, v_j)\;,
\end{equation}
where $w_{u_i}$ and $w_{v_j}$ represent the weights (probabilities)  of the corresponding generator $u_i$ and discriminator $v_j$ with respect to the $N$-component mixtures. The objective is minimized using backpropagation. Moreover, the weights are regularized such that they are not too far away from uniform. 

\begin{comment}
At every iteration, Algorithm~\ref{alg:coev-gan} optimizes, with respect to $\{u_i\}$ and $\{v_j\}$, the following objective function
 \begin{equation}
 \label{eq:lipz-gan}
 \min_{\{u_i\}} \max_{\{v_j\}}\sum^{T}_{i=1} \sum^{T}_{j=1}  x_{ij} \calL(u_i, v_j)\;, \text{where}
 \end{equation}
\[
x_{ij} = 
\begin{cases}
1\;, & \text{with probability}\;\; p_{ij}; \\
0\;, & \text{otherwise.} \\
\end{cases}
\]When $p_{ij}=w_{u_i} w_{v_j}$, the summation in ~\eqref{eq:mix-gan} is the expectation of that in~\eqref{eq:lipz-gan}.
\end{comment}

Our proposition (Algorithm~\ref{alg:adv-coev-gan}) solves multiple distributed instances (one per neighborhood) of the objective function~\eqref{eq:mix-gan} (Lines~\ref{line:parfor-beg} to~\ref{line:parfor-end} of Algorithm~\ref{alg:adv-coev-gan}) where the weights of both populations are set to uniform (as effected by the non-weighted sum of the fitness value in Lines~\ref{line:fit-update-beg} and~\ref{line:fit-update-end} of Algorithm~\ref{alg:basic-coev-gan}). At the same time, an optimal mixture of generators over the population is learnt in an evolutionary fashion using the desired performance metric (Line~\ref{line:es} of Algorithm~\ref{alg:adv-coev-gan}), without the need for a mixture of \emph{discriminators}. Besides spatial coevolution, this hierarchical separation between the generator and discriminator neural net parameters on one side and the generators mixture weights on the other side is one of the main differences between our proposition and that of~\cite{arora2017generalization}. Note that it is possible to incorporate \cite{arora2017generalization}'s in our distributed coevolutionary framework by introducing weights for the discriminators and making the fitness values (Lines~\ref{line:fit-update-beg} and~\ref{line:fit-update-end} of Algorithm~\ref{alg:basic-coev-gan}) weighted by $w_{u_i}$ and $w_{v_j}$. Consequently, both the generator and discriminator mixture weights can be updated within the spatial coevolution framework (Lines~\ref{line:parfor-beg} to~\ref{line:parfor-end} of Algorithm~\ref{alg:adv-coev-gan}) in contrast to our main proposition of learning only the generator mixture weights in tandem with the spatial coevolution framework (Line~\ref{line:es} of Algorithm~\ref{alg:adv-coev-gan}). In our experiments, we report results for both variants, which we refer to by \horse (without discriminator mixture weights) and \horsed (with discriminator mixture weights).


